NIKI: Neural Inverse Kinematics with Invertible Neural Networks for 3D Human Pose and Shape Estimation

With the progress of 3D human pose and shape estimation, state-of-the-art methods can either be robust to occlusions or obtain pixel-aligned accuracy in non-occlusion cases. However, they cannot obtain robustness and mesh-image alignment at the same time. In this work, we present NIKI (Neural Inverse Kinematics with Invertible Neural Network), which models bi-directional errors to improve the robustness to occlusions and obtain pixel-aligned accuracy. NIKI can learn from both the forward and inverse processes with invertible networks. In the inverse process, the model separates the error from the plausible 3D pose manifold for a robust 3D human pose estimation. In the forward process, we enforce the zero-error boundary conditions to improve the sensitivity to reliable joint positions for better mesh-image alignment. Furthermore, NIKI emulates the analytical inverse kinematics algorithms with the twist-and-swing decomposition for better interpretability. Experiments on standard and occlusion-specific benchmarks demonstrate the effectiveness of NIKI, where we exhibit robust and well-aligned results simultaneously. Code is available at https://github.com/Jeff-sjtu/NIKI

==> sections/methodbak.tex <==
\section{Method}

In this section, we present NIKI, a neural inverse kinematics solution for 3D human pose and shape estimation. We first review the formulation of existing analytical and MLP-based IK algorithms in \S\ref{sec:ik}. In \S\ref{sec:ik_inn}, we present the formulation of the proposed INN-based IK algorithm with bi-directional error decoupling. In \S\ref{sec:arch}, we elaborate on the proposed IK-specific invertible architecture. Then we present the overall pose estimation framework and the training losses in \S\ref{sec:train}. Finally, we provide the necessary implementation details in \S\ref{sec:implement}

\subsection{Preliminaries}
\label{sec:ik}
% 1. ik, fk; 2. inn; 3. information perserved, error decoupling;

% We study the problem of inverse kinematics (IK) using invertible neural networks (INNs).
The IK process is to find the corresponding body part rotations that explain the input body joint positions, while the forward kinematics (FK) process computes the desired joint positions based on the input rotations. The FK process is well-defined, but the transformation from joint rotations to joint positions incurs an information loss, resulting in the ill-posed IK process. Here, we follow HybrIK~\cite{li2021hybrik} to consider twist rotations for information integrity.

\begin{figure}[tbp]
    \centering
    % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{figures/decoupling.pdf}
 
    \caption{\textbf{Illustration} of (a) analytical IK, (b) feedforward MLP-based IK, and (c) NIKI with bi-directional error decoupling.}
    \label{fig:decouple}
\end{figure}

The conventional IK algorithms only require the output rotations to match the input joint positions but ignore the errors of the joint positions and the plausibility of the body pose. Therefore, the errors of the joint positions will propagate to the joint rotations (Fig.~\ref{fig:decouple}a). This process can be formulated as:
\begin{equation}
    \mathbf{R} + \epsilon_r = \text{IK}(\mathbf{p} + \epsilon_p, \boldsymbol{\phi} + \epsilon_{\phi} ~|~ \boldsymbol{\beta}),
\end{equation}
where $\mathbf{R}$ denotes the rotations of body parts, $\epsilon_r$ denotes the propagated error of the rotations, $\mathbf{p}$ denotes the underlying plausible joint positions, $\epsilon_p$ denotes the position errors, $\boldsymbol{\phi}$ denotes the underlying plausible twist rotations, $\epsilon_{\phi}$ denotes the twist error, and $\boldsymbol{\beta}$ denotes the body shape parameters.

A straightforward solution to improve the robustness of the IK algorithms is using the standard regression model~\cite{csiszar2017solving,zhang2020object} to output the underlying plausible rotations given the erroneous input (Fig.~\ref{fig:decouple}b):
% To improve the robustness of the IK process to joint position and twist rotation errors, a straightforward solution is to train a standard regression model~\cite{csiszar2017solving,zhang2020object} to output the underlying plausible rotations given deviated input (Fig.~\ref{fig:decouple}b):
\begin{equation}
    \mathbf{R} = \text{IK}(\mathbf{p} + \epsilon_p, \boldsymbol{\phi} + \epsilon_{\phi} ~|~ \boldsymbol{\beta}).
\end{equation}
% As shown in Fig.~\ref{fig:decouple}(b), the model can be trained to predict the correct rotations with erroneous input.  
Indeed, modeling the IK process with classical neural networks, \eg, MLP, can improve the robustness. However, it makes the output rotations less sensitive to the change of the joint positions. The errors are highly coupled with the joint positions. Without explicit decoupling, it is difficult for the network to distinguish between the valid change of the joint positions and the deviation from the manifold of plausible human poses. Therefore, the output rotations cannot accurately track the movement of the body joints. In practice, we find that the feedforward neural networks could improve performance in occluded scenes but cause performance degradation in non-occlusion scenes, where accurate mesh-image alignment is required.

\subsection{Inverse Kinematics with INNs}
\label{sec:ik_inn}
In this work, to improve the robustness of IK to occlusions while maintaining the sensitivity to non-occluded body joints, we propose to use the invertible neural network (INN) to model bi-directional errors explicitly (see Fig.~\ref{fig:decouple}c). In contrast to the conventional methodology, we learn model $g(\cdot ; \boldsymbol{\beta}, \theta)$ of the IK process jointly with model $f(\cdot ; \boldsymbol{\beta}, \theta)$ approximating the FK process:
\begin{align}
    [\mathbf{p} + \epsilon_p, \boldsymbol{\phi} + \epsilon_{\phi}] &= f(\mathbf{R}, \mathbf{z}_r ; \boldsymbol{\beta}, \theta), \\
    [\mathbf{R}, \mathbf{z}_r] &= g(\mathbf{p} + \epsilon_p, \boldsymbol{\phi} + \epsilon_{\phi} ; \boldsymbol{\beta}, \theta),
\end{align}
where $\mathbf{z}_r$ is the latent error embedding that denotes how the input joint positions deviate from the manifold of plausible human poses. Notice that $f$ and $g$ share the same parameters $\theta$, and $f=g^{-1}$ is enforced by the invertible network architecture. Thus simultaneously learning the FK and IK processes can benefit each other.

In the forward process, we can tune the error embedding $\mathbf{z}_r$ to control the error level of the body joint positions. The body part rotations can keep sensitive to the movement of body joint positions by setting $\mathbf{z}_r$ to $0$, which means no deviation from the pose manifold, and the rotations should perfectly match the joint positions. In the inverse process, the output rotations are robust to the erroneous input. The deviation from the manifold only reflects on $\mathbf{z}_r$ while the rotation $\mathbf{R}$ keeps stable.

\paragraph{Decouple Error Information.}
To model the errors in both forward and inverse directions, we need to separate the error information from the pose information. The total information of the input contains two parts: i) the pose information that lies on the manifold of plausible poses; ii) the error information that indicates how the input deviates from the manifold. Since the invertible network establishes a bijective mapping, all the input information will be preserved in the output. Additionally, no new information will be introduced.
% This is the basis of error decoupling.
To obtain the error information, we only need to let $\mathbf{R}$ learn the human poses and remove the pose information in the output vector $\mathbf{z}_r$. The vector $\mathbf{z}_r$ will automatically encode the remaining error information. Concretely, we enforce $\mathbf{R}$ and $\mathbf{z}_r$ to be independent upon convergence, \ie, $p(\mathbf{z}_r | \mathbf{R}) = p(\mathbf{z}_r)$, to remove the pose information from $\mathbf{z}_r$. Besides, the model needs to satisfy the following zero-error conditions to maintain sensitivity to error-free body joint positions:
% To decouple the errors, the latent code $\mathbf{z}_r$ should have no pose information.
% we train the bijective mapping to satisfy the following the zero-error conditions:
\begin{align}
    [\mathbf{p}, \phi] &= f(\mathbf{R}, \bigzero ; \boldsymbol{\beta}, \theta), \\
    [\mathbf{R}, \bigzero] &= g(\mathbf{p}, \boldsymbol{\phi} ; \boldsymbol{\beta}, \theta).
\end{align}
With the independence and zero-error constraints, the network is able to model the error information in the forward and inverse process.
% With the constraints for the zero-error boundary, we explicitly let the model decouple the bi-directional errors.
% In the forward process, we can tune error embedding $\mathbf{z}_r$ to control the error level of the body joint positions. The body part rotations can keep sensitive to the movement of body joint positions by setting $\mathbf{z}_r$ to $0$. In the inverse process, the error decoupling makes the output rotations stable and robust to the erroneous input.

% The error decoupling in the inverse process makes the model robust to input errors, while the error modeling in the forward process keeps the body part rotations sensitive to the movement of error-free body joint positions.

\subsection{Invertible Architecture}
\label{sec:arch}

\paragraph{One-Stage Mapping.}
To build a fully invertible neural network for inverse kinematics, we build the one-stage mapping model using RealNVP~\cite{dinh2016density}. Since the IK and FK processes need to know the skeleton length, we extend the INN to incorporate the conditional shape parameters input. The basic block of the network contains two reversible coupling layers. The input vector $\mathbf{u}$ of the block is split into two parts, $\mathbf{u}_1$ and $\mathbf{u}_2$, which are subsequently transformed with coefficients $\exp(s_i)$ and $t_i$ ($i \in \{1, 2\}$) by the two affine coupling layers:
\begin{align}
    \mathbf{v}_1 = \mathbf{u}_1 \odot \exp(s_2(\mathbf{u}_2, \boldsymbol{\beta})) + t_2(\mathbf{u}_2, \boldsymbol{\beta}), \label{eq:affine1}\\
    \mathbf{v}_2 = \mathbf{u}_2 \odot \exp(s_1(\mathbf{v}_1, \boldsymbol{\beta})) + t_1(\mathbf{v}_1, \boldsymbol{\beta}), \label{eq:affine2}
\end{align}
where $\mathbf{v} = [\mathbf{v}_1, \mathbf{v}_2]$ is the output vector of the block and $\odot$ denotes element-wise multiplication. The coefficients of the affine transformation can be learned by arbitrarily complex functions, which do not need to be invertible. The invertibility is guaranteed by the affine transformation in Eq.~\ref{eq:affine1} and \ref{eq:affine2}.
The overall network consists of multiple blocks connected in series to increase capacity.
% To increase capacity, the overall network consists of multiple block connect in stack.
Besides, since the invertible network requires the input and output vectors have the same dimension, we follow previous work~\cite{ardizzone2018analyzing} and pad zeros to the input.


% \begin{figure}[t]
%     \centering
%     % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%     \includegraphics[width=0.8\linewidth]{figures/arch.pdf}
 
%     \caption{\textbf{Twist-and-Swing mapping.}}
%     \label{fig:arch}
% \end{figure}

\paragraph{Twist-and-Swing Mapping.}
Although treating the invertible neural network as a black box can model both the FK and IK processes at the same time, we further emulate the analytical IK algorithm to improve the model performance. Specifically, we follow the twist-and-swing composition~\cite{li2021hybrik} and divide the IK process into two steps: i) joint positions to swing rotations;  ii) twist and swing rotations to complete rotations. The two-step mapping is finished by two separate invertible neural networks:
\begin{align}
    [\mathbf{R}_{\textit{sw}}, \mathbf{z}_{\textit{sw}}] &= g_1(\mathbf{p} + \epsilon_p ; \boldsymbol{\beta}, \theta_1), \\
    [\mathbf{R}, \mathbf{z}_r] &= g_2(\mathbf{R}_{\textit{sw}} ,\boldsymbol{\phi} + \epsilon_{\phi} ; \theta_2),
\end{align}
where $\mathbf{R}_{\textit{sw}}$ is the swing rotations, and $\mathbf{z}_{\textit{sw}}$ indicates the deviation from the plausible swing rotation manifold.
% The first step uses a conditional invertible network, which takes as input the noisy joint positions $\mathbf{p} + \epsilon_p$ with the shape condition $\boldsymbol{\beta}$ and predict the swing rotations $\mathbf{R}_{\textit{sw}}$ and the error of swing rotations $\mathbf{z}_{\textit{sw}}$. The second step uses a invertible network without conditions.
% It maps the swing rotations $\mathbf{R}_{\textit{sw}}$ and the twist rotations $\boldsymbol{\phi}$ to the complete rotations $\mathbf{R}$ and the latent embedding $\mathbf{z}_{\text{r}}$ that denotes the error of the complete rotations, which further includes the implausible twisting information.
% The whole process of the twist-and-swing mapping is illustrated in Fig.~\ref{fig:arch}(b).

Such two-step twist-and-swing mapping improves the interpretability of the IK network. Besides, since the mappings are bijective, the FK process also follows the twist-and-swing procedure but inversely. We have $f = f_1 \odot f_2 = g_1^{-1} \odot g_2^{-1} = g^{-1}$. In the FK process, the body part rotations are first decomposed into twist and swing rotations. Then the swing rotations are transformed into the joint positions.

\paragraph{Temporal Extension.}
The invertible framework is flexible. It can be easily extended to temporal input and incorporate motion information to solve the IK problem. The model with static input can only identify the errors related to physiological implausibility, while the temporal model can further improve motion smoothness by decoupling errors of implausible body movements. More details and experimental results are provided in the supplementary material.
% (TODO: model architecture)

\begin{figure}[t]
    \centering
    % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{figures/framework.pdf}
 
    \caption{\textbf{Overview of the proposed framework.} The input image is fed into the CNN backbone network to estimate the initial joint positions and twist rotations, followed by NIKI to solve the joint rotations.}
    \label{fig:framework}
 \end{figure}

\subsection{Decoupled Learning}
\label{sec:train}

The overview of our approach is illustrated in Fig.~\ref{fig:framework}. During inference, we first extract the joint positions and twist rotations, which are subsequently fed to the invertible network to predict the complete body part rotations.
During training, we can optimize FK and IK simultaneously in one network.
% During training, the invertible neural network allows us to simultaneously optimize FK and IK to train the same network.
Hereby, we perform FK and IK alternately with the additional independence loss and boundary loss. The gradients from both directions are accumulated before performing a parameter update.

\paragraph{Inverse Training.}
In the inverse iteration, the network predicts the body part rotations given the joint positions and twist rotations. The loss function is defined as:
\begin{equation}
    \mathcal{L}^{\textit{inv}}_{\textit{rot}} = \big\| \hat{\mathbf{R}}^{\textit{inv}} - \widetilde{\mathbf{R}} \big\|^2_2 + \big\| \text{FK}(\hat{\mathbf{R}}^{\textit{inv}}) - \text{FK}(\widetilde{\mathbf{R}}) \big\|_1,
    \label{eq:inv_r}
\end{equation}
with
\begin{equation}
    [\hat{\mathbf{R}}^{\textit{inv}}, \hat{\mathbf{z}}_r] = g(\hat{\mathbf{p}}, \hat{\boldsymbol{\phi}} ; \boldsymbol{\beta}, \theta),
\end{equation}
where $\hat{\mathbf{p}}$ and $\hat{\boldsymbol{\phi}}$ denote the noisy predictions from the CNN backbone, $\widetilde{\mathbf{R}}$ represents the ground-truth rotations, and $\text{FK}(\cdot)$ denotes the analytical FK process to supervise corresponding the 3D joint positions of predicted pose. For the twist-and-swing mapping model, we additionally supervise the swing rotations:
\begin{equation}
    \mathcal{L}^{\textit{inv}}_{\textit{sw}} = \big\| \hat{\mathbf{R}}^{\textit{inv}}_{\textit{sw}} - \widetilde{\mathbf{R}}_{\textit{sw}} \big\|^2_2,
\end{equation}
with
\begin{equation}
    [\hat{\mathbf{R}}^{\textit{inv}}_{\textit{sw}}, \hat{\mathbf{z}}_\textit{sw}] = g_1(\hat{\mathbf{p}} ; \boldsymbol{\beta}, \theta_1).
\end{equation}
% where $\hat{\mathbf{R}}^{\textit{sw}}$ represents the ground-truth swing rotations.

\paragraph{Forward Training.}
In the forward process, the network predicts the joint positions and twist rotations given the body part rotations. The error of the noisy predictions from the CNN backbone should only depend on the error embedding. Therefore, with the ground-truth rotations and error embedding $\hat{\mathbf{z}}_r$ obtained from the inverse iteration, the forward model should predict the same values as the CNN output:
\begin{equation}
    \mathcal{L}^{\textit{fwd}} = \| \hat{\mathbf{p}}^{\textit{fwd}} - \hat{\mathbf{p}} \|_1 + \| \hat{\boldsymbol{\phi}}^{\textit{fwd}} - \hat{\boldsymbol{\phi}} \|_2^2,
\end{equation}
with
\begin{equation}
    [\hat{\mathbf{p}}^{\textit{fwd}}, \hat{\boldsymbol{\phi}}^{\textit{fwd}}] = f(\widetilde{\mathbf{R}}, \hat{\mathbf{z}}_r ; \boldsymbol{\beta}, \theta).
\end{equation}
For the twist-and-swing mapping model, we also supervise the swing rotations:
\begin{equation}
    \mathcal{L}^{\textit{fwd}}_{\textit{sw}} = \big\| \hat{\mathbf{R}}^{\textit{fwd}}_{\textit{sw}} - \hat{\mathbf{R}}^{\textit{inv}}_{\textit{sw}} \big\|^2_2,
\end{equation}
with
\begin{equation}
    [\hat{\mathbf{R}}^{\textit{fwd}}_{\textit{sw}}, \hat{\boldsymbol{\phi}}^{\textit{fwd}}] = f_2(\widetilde{\mathbf{R}}, \mathbf{z}_r ; \theta_2).
\end{equation}

\paragraph{Independence Loss.}
% The characteristic of bijective mappings ensure that there is no information loss in both the forward and inverse transformations. When the input contains the pose information and the error information, the output must contain the same information. This is the basis of the error decoupling process.

% The latent error vector denotes how the joint positions deviate from the manifold of plausible human poses.

% which is difficult to define and learn in a supervised manner. Since the total amount of information is constant, we can enforce $\mathbf{z}_r$ to contain error information by supervising the inverse output $\mathbf{R}_{\textit{inv}}$ with pose rotations and
The latent error vector is learned in an unsupervised manner by making $\mathbf{R}_{\textit{inv}}$ and $\mathbf{z}_r$ independent of each other. The pose information is supervised by Eq.~\ref{eq:inv_r}. We then enforce the independence by penalizing the mismatch between the joint distribution of the rotations and error embedding $q\big(\hat{\mathbf{R}}^{\textit{inv}}, \mathbf{z}_r\big)$ and the product of marginal distributions $p\big(\widetilde{\mathbf{R}} \big)p(\mathbf{z})$:
\begin{equation}
    \mathcal{L}_{\textit{ind}} = \mathcal{D}(q\big(\mathbf{R}^{\textit{inv}}, \mathbf{z}_r\big), p\big(\widetilde{\mathbf{R}} \big)p(\mathbf{z})),
\end{equation}
where $\mathbf{z} \sim \mathcal{N}(0, \mathbf{I})$ follows the standard normal distribution, $\mathbf{I}$ is the identity matrix, and $\mathcal{D}(\cdot)$ denotes the Maximum Mean Discrepancy~\cite{gretton2012kernel}, which allows us to compare two probability distributions through samples. $\mathcal{L}_{\textit{ind}}$ not only makes $\mathbf{R}^{\textit{inv}}$ and $\mathbf{z}_r$ independent but also enforces the error embedding $\mathbf{z}_r$ to follow the standard normal distribution $p(\mathbf{z})$, serving as a regularization.

\paragraph{Boundary Condition Loss.}
To enforce the solved rotations to explain the reliable joint positions, we supervise the boundary cases where no errors occur. In the inverse process, the output error should be zero when the network is input with ground truth:
\begin{equation}
    \mathcal{L}^{\textit{inv}}_{\textit{bnd}} = \| \hat{\epsilon}_r \|_2^2 + \| \hat{\mathbf{R}}^{\textit{bnd}} - \widetilde{\mathbf{R}} \|^2_2,
\end{equation}
with
\begin{equation}
    [\hat{\mathbf{R}}^{\textit{bnd}}, \hat{\epsilon}_r] = g(\widetilde{\mathbf{p}}, \widetilde{\boldsymbol{\phi}} ; \boldsymbol{\beta}, \theta).
\end{equation}
% For the twist-and-swing mapping model, we also supervise the error embedding of the swing rotations.
% \begin{equation}
%     \mathcal{L}^{\textit{inv}}_{\textit{bnd},\textit{sw}} = \| \epsilon_{\textit{sw}} \|_2^2, 
% \end{equation}
% with
% \begin{equation}
%     [\mathbf{R}_{\textit{bnd}}^{\textit{sw}}, \epsilon_{\textit{sw}}] = g_1(\widetilde{\mathbf{p}}, \widetilde{\boldsymbol{\phi}} ; \boldsymbol{\beta}, \theta_1).
% \end{equation}
In the forward process, the joint positions and twist rotations should map to the ground truth when the error vector $\mathbf{z}_r$ is $\mathbf{0}$:
\begin{equation}
    \mathcal{L}^{\textit{fwd}}_{\textit{bnd}} = \| \hat{\mathbf{p}}^{\textit{bnd}} - \widetilde{\mathbf{p}} \|_1 + \| \hat{\boldsymbol{\phi}}^{\textit{bnd}} - \widetilde{\boldsymbol{\phi}} \|_2^2,
\end{equation}
with
\begin{equation}
    [\hat{\mathbf{p}}^{\textit{bnd}}, \hat{\boldsymbol{\phi}}^{\textit{bnd}}] = f(\widetilde{\mathbf{R}}, \mathbf{0} ; \boldsymbol{\beta}, \theta).
\end{equation}

\subsection{Implementation Details.}
\label{sec:implement}

We adopt HybrIK~\cite{li2021hybrik} as the CNN backbone to predict the noisy body joint positions and the twist rotations.
The input of the IK model includes the joint positions $\mathbf{p} \in \mathbb{R}^{3K}$, twist rotations parameterized in 2-dimensional vectors for each joint, \ie, $\boldsymbol{\phi} \in \mathbb{R}^{2(K - 1)}$, and the confidence scores of each joint $\mathbf{s} \in \mathbb{R}^{K}$, where $K$ denotes the total number of human body joints. The total valid dimension of the input is $D_{\textit{in}} = 6K - 2$. The output of the model consists of the body part rotations parameterized as a 6D vector for each part, \ie, $\mathbf{R} \in \mathbb{R}^{6K}$, and the error embedding $\mathbf{z}_r \in \mathbb{R}^{D_z}$. Therefore, the valid output dimension is $D_{\textit{out}} = 6K + D_z$. Since $D_{\textit{out}} > D_{\textit{in}}$, we pad the input with a zero vector with the dimension $M = D_{\textit{out}} - D_{\textit{in}} = D_z + 2$ to satisfy the constraints of the invertible neural network.

% The input of the direct mapping IK model contains the joint positions $\mathbf{p} \in \mathbb{R}^{3K}$, twist rotations parameterized in 2-dimensional vectors for each joint, \ie, $\boldsymbol{\phi} \in \mathbb{R}^{2(K - 1)}$, and the confidence scores of each joints $\mathbf{s} \in \mathbb{R}^{K}$, where $K$ denotes the total number of human body joints. The total valid dimension of the input is $D_{\textit{in}} = 6K - 2$. The output of the model consists of the body part rotations parameterized as a 6D vector for each part, \ie, $\mathbf{R} \in \mathbb{R}^{6K}$, and the error embedding $\epsilon_r \in \mathbb{R}^{D_\epsilon}$. Therefore, the valid output dimension is $D_{\textit{out}} = 6K + D_{\epsilon}$. Since $D_{\textit{out}} > D_{\textit{in}}$, we pad the input of the direct mapping network with a zero vector with the dimension $M = D_{\textit{out}} - D_{\textit{in}} = D_{\epsilon} + 2$, to satisfy the constraints of the invertible neural network.

% For the twist-and-swing mapping model, the input to the first network are the joint positions $\mathbf{p}$ and confidence scores $\mathbf{s}$. The intermediate outputs are the swing rotations $\mathbf{R}^{\textit{sw}} \in \mathbb{R}^{6K}$ and the error embedding for the swing rotations $\epsilon_{s} \in \mathbb{R}^{32}$. Therefore, the input to the first network is padded with a zero vector, of which the dimension is $2K + D_{\epsilon}$. The input to the second network are swing and twist rotations, while the output are the complete rotations $\mathbf{R}$ and the error embedding $\epsilon_r \in \mathbb{R}^{D_{\epsilon}}$. We set $D_{\epsilon}$ to $2(K - 1)$ and thus the input of the second network does not require zero-paddings.

The networks are trained with Adam solver for 50 epochs with a mini-batch size of $64$. The learning rate is set to $1 \times 10^{-3}$ at first and reduced by a factor of 10 at the 30th and 40th epochs.
Implementation details and experimental results of the temporal NIKI are provided in the supplementary material.
% Implementation is in PyTorch.

